SimAb: A simple, fast and flexible model to assess the effects of planet formation on the atmospheric composition of gas giants

We present a basic, fast, and flexible planet formation model, called SimAb (Simulating Abundances), to form giant planets and study their primary atmospheric composition soon after their formation. In SimAb we introduce parameters to simplify the assumptions about the complex physics involved in the formation of a planet. This approach allows us to trace and understand the influence of complex physical processes on the formed planets. We focus on the C/O ratio and the metallicity of the planetary atmosphere as an indicator of their compositions. We show that the initial protoplanet core mass does not influence the final composition of the planetary atmosphere in the context of our model. The initial orbital distance affects the C/O ratio due to the different C/O ratios in the gas phase and the solid phase at different orbital distances. Additionally, the initial orbital distance together with the amount of accreted planetesimals cause the planet to have sub-solar or super-solar metallicity. Furthermore, the C/O ratio is affected by the dust grain fraction and the planetesimal fraction. Planets that accrete most of their heavy elements through dust grains will have a C/O ratio close to the solar C/O ratio, while planets that accrete most of their heavy elements from the planetesimals in the disk will end up with a C/O ratio closer to the C/O ratio in the solid phase of the disk. By using the C/O ratio and metallicity together we can put a lower and upper boundary on the initial orbital distance where super-solar metallicity planets are formed. We show that planetesimals are the main source for reaching super-solar metallicity planets. On the other hand, planets that mainly accrete dust grains will show a more solar composition. Super-solar metallicity planets that initiate their formation farther than the CO ice line have a C/O ratio closer to the solar value.

==> reference.tex <==
@ARTICLE{Alibert_2005,
	author = {{Alibert}, Yann and {Mordasini}, Christoph and {Mousis}, Olivier and
	{Benz}, Willy},
	title = "{Formation of Giant Planets  An Attempt in Matching Observational Constraints}",
	journal = {Space Science Reviews},
	keywords = {Stars: planetary systems, stars: planetary systems, formation-solar system, formation},
	year = 2005,
	month = jan,
	volume = {116},
	number = {1-2},
	pages = {77-95},
	doi = {10.1007/s11214-005-1949-z},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2005SSRv..116...77A},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{AliDib_2014,
   title={CARBON-RICH PLANET FORMATION IN A SOLAR COMPOSITION DISK},
   volume={785},
   ISSN={1538-4357},
   url={http://dx.doi.org/10.1088/0004-637X/785/2/125},
   DOI={10.1088/0004-637x/785/2/125},
   number={2},
   journal={The Astrophysical Journal},
   publisher={IOP Publishing},
   author={Ali-Dib, Mohamad and Mousis, Olivier and Petit, Jean-Marc and Lunine, Jonathan I.},
   year={2014},
   month={Apr},
   pages={125}
}
@ARTICLE{ARIEL,
       author = {{Tinetti}, Giovanna and {Drossart}, Pierre and {Eccleston}, Paul and {Hartogh}, Paul and {Heske}, Astrid and {Leconte}, J{\'e}r{\'e}my and {Micela}, Giusi and {Ollivier}, Marc and {Pilbratt}, G{\"o}ran and {Puig}, Ludovic and {Turrini}, Diego and {Vandenbussche}, Bart and {Wolkenberg}, Paulina and {Beaulieu}, Jean-Philippe and {Buchave}, Lars A. and {Ferus}, Martin and {Griffin}, Matt and {Guedel}, Manuel and {Justtanont}, Kay and {Lagage}, Pierre-Olivier and {Machado}, Pedro and {Malaguti}, Giuseppe and {Min}, Michiel and {N{\o}rgaard-Nielsen}, Hans Ulrik and {Rataj}, Mirek and {Ray}, Tom and {Ribas}, Ignasi and {Swain}, Mark and {Szabo}, Robert and {Werner}, Stephanie and {Barstow}, Joanna and {Burleigh}, Matt and {Cho}, James and {du Foresto}, Vincent Coud{\'e} and {Coustenis}, Athena and {Decin}, Leen and {Encrenaz}, Therese and {Galand}, Marina and {Gillon}, Michael and {Helled}, Ravit and {Morales}, Juan Carlos and {Mu{\~n}oz}, Antonio Garc{\'\i}a and {Moneti}, Andrea and {Pagano}, Isabella and {Pascale}, Enzo and {Piccioni}, Giuseppe and {Pinfield}, David and {Sarkar}, Subhajit and {Selsis}, Franck and {Tennyson}, Jonathan and {Triaud}, Amaury and {Venot}, Olivia and {Waldmann}, Ingo and {Waltham}, David and {Wright}, Gillian and {Amiaux}, Jerome and {Augu{\`e}res}, Jean-Louis and {Berth{\'e}}, Michel and {Bezawada}, Naidu and {Bishop}, Georgia and {Bowles}, Neil and {Coffey}, Deirdre and {Colom{\'e}}, Josep and {Crook}, Martin and {Crouzet}, Pierre-Elie and {Da Peppo}, Vania and {Sanz}, Isabel Escudero and {Focardi}, Mauro and {Frericks}, Martin and {Hunt}, Tom and {Kohley}, Ralf and {Middleton}, Kevin and {Morgante}, Gianluca and {Ottensamer}, Roland and {Pace}, Emanuele and {Pearson}, Chris and {Stamper}, Richard and {Symonds}, Kate and {Rengel}, Miriam and {Renotte}, Etienne and {Ade}, Peter and {Affer}, Laura and {Alard}, Christophe and {Allard}, Nicole and {Altieri}, Francesca and {Andr{\'e}}, Yves and {Arena}, Claudio and {Argyriou}, Ioannis and {Aylward}, Alan and {Baccani}, Cristian and {Bakos}, Gaspar and {Banaszkiewicz}, Marek and {Barlow}, Mike and {Batista}, Virginie and {Bellucci}, Giancarlo and {Benatti}, Serena and {Bernardi}, Pernelle and {B{\'e}zard}, Bruno and {Blecka}, Maria and {Bolmont}, Emeline and {Bonfond}, Bertrand and {Bonito}, Rosaria and {Bonomo}, Aldo S. and {Brucato}, John Robert and {Brun}, Allan Sacha and {Bryson}, Ian and {Bujwan}, Waldemar and {Casewell}, Sarah and {Charnay}, Bejamin and {Pestellini}, Cesare Cecchi and {Chen}, Guo and {Ciaravella}, Angela and {Claudi}, Riccardo and {Cl{\'e}dassou}, Rodolphe and {Damasso}, Mario and {Damiano}, Mario and {Danielski}, Camilla and {Deroo}, Pieter and {Di Giorgio}, Anna Maria and {Dominik}, Carsten and {Doublier}, Vanessa and {Doyle}, Simon and {Doyon}, Ren{\'e} and {Drummond}, Benjamin and {Duong}, Bastien and {Eales}, Stephen and {Edwards}, Billy and {Farina}, Maria and {Flaccomio}, Ettore and {Fletcher}, Leigh and {Forget}, Fran{\c{c}}ois and {Fossey}, Steve and {Fr{\"a}nz}, Markus and {Fujii}, Yuka and {Garc{\'\i}a-Piquer}, {\'A}lvaro and {Gear}, Walter and {Geoffray}, Herv{\'e} and {G{\'e}rard}, Jean Claude and {Gesa}, Lluis and {Gomez}, H. and {Graczyk}, Rafa{\l} and {Griffith}, Caitlin and {Grodent}, Denis and {Guarcello}, Mario Giuseppe and {Gustin}, Jacques and {Hamano}, Keiko and {Hargrave}, Peter and {Hello}, Yann and {Heng}, Kevin and {Herrero}, Enrique and {Hornstrup}, Allan and {Hubert}, Benoit and {Ida}, Shigeru and {Ikoma}, Masahiro and {Iro}, Nicolas and {Irwin}, Patrick and {Jarchow}, Christopher and {Jaubert}, Jean and {Jones}, Hugh and {Julien}, Queyrel and {Kameda}, Shingo and {Kerschbaum}, Franz and {Kervella}, Pierre and {Koskinen}, Tommi and {Krijger}, Matthijs and {Krupp}, Norbert and {Lafarga}, Marina and {Landini}, Federico and {Lellouch}, Emanuel and {Leto}, Giuseppe and {Luntzer}, A. and {Rank-L{\"u}ftinger}, Theresa and {Maggio}, Antonio and {Maldonado}, Jesus and {Maillard}, Jean-Pierre and {Mall}, Urs and {Marquette}, Jean-Baptiste and {Mathis}, Stephane and {Maxted}, Pierre and {Matsuo}, Taro and {Medvedev}, Alexander and {Miguel}, Yamila and {Minier}, Vincent and {Morello}, Giuseppe and {Mura}, Alessandro and {Narita}, Norio and {Nascimbeni}, Valerio and {Nguyen Tong}, N. and {Noce}, Vladimiro and {Oliva}, Fabrizio and {Palle}, Enric and {Palmer}, Paul and {Pancrazzi}, Maurizio and {Papageorgiou}, Andreas and {Parmentier}, Vivien and {Perger}, Manuel and {Petralia}, Antonino and {Pezzuto}, Stefano and {Pierrehumbert}, Ray and {Pillitteri}, Ignazio and {Piotto}, Giampaolo and {Pisano}, Giampaolo and {Prisinzano}, Loredana and {Radioti}, Aikaterini and {R{\'e}ess}, Jean-Michel and {Rezac}, Ladislav and {Rocchetto}, Marco and {Rosich}, Albert and {Sanna}, Nicoletta and {Santerne}, Alexandre and {Savini}, Giorgio and {Scandariato}, Gaetano and {Sicardy}, Bruno and {Sierra}, Carles and {Sindoni}, Giuseppe and {Skup}, Konrad and {Snellen}, Ignas and {Sobiecki}, Mateusz and {Soret}, Lauriane and {Sozzetti}, Alessandro and {Stiepen}, A. and {Strugarek}, Antoine and {Taylor}, Jake and {Taylor}, William and {Terenzi}, Luca and {Tessenyi}, Marcell and {Tsiaras}, Angelos and {Tucker}, C. and {Valencia}, Diana and {Vasisht}, Gautam and {Vazan}, Allona and {Vilardell}, Francesc and {Vinatier}, Sabrine and {Viti}, Serena and {Waters}, Rens and {Wawer}, Piotr and {Wawrzaszek}, Anna and {Whitworth}, Anthony and {Yung}, Yuk L. and {Yurchenko}, Sergey N. and {Osorio}, Mar{\'\i}a Rosa Zapatero and {Zellem}, Robert and {Zingales}, Tiziano and {Zwart}, Frans},
        title = "{A chemical survey of exoplanets with ARIEL}",
      journal = {Experimental Astronomy},
     keywords = {Exoplanets, Space missions, IR spectroscopy, Molecular signatures},
         year = 2018,
        month = nov,
       volume = {46},
       number = {1},
        pages = {135-209},
          doi = {10.1007/s10686-018-9598-x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ExA....46..135T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Asplund_2009,
   title={The Chemical Composition of the Sun},
   volume={47},
   ISSN={1545-4282},
   url={http://dx.doi.org/10.1146/annurev.astro.46.060407.145222},
   DOI={10.1146/annurev.astro.46.060407.145222},
   number={1},
   journal={Annual Review of Astronomy \& Astrophysics},
   publisher={Annual Reviews},
   author={Asplund, Martin and Grevesse, Nicolas and Sauval, A. Jacques and Scott, Pat},
   year={2009},
   month={Sep},
   pages={481–522}
}


@ARTICLE{Baruteau_2014,
	author = {{Baruteau}, C. and {Crida}, A. and {Paardekooper}, S.-J. and 
	{Masset}, F. and {Guilet}, J. and {Bitsch}, B. and {Nelson}, R. and 
	{Kley}, W. and {Papaloizou}, J.},
	title = "{Planet-Disk Interactions and Early Evolution of Planetary Systems}",
	journal = {Protostars and Planets VI},
	archivePrefix = "arXiv",
	eprint = {1312.4293},
	primaryClass = "astro-ph.EP",
	year = 2014,
	pages = {667-689},
	doi = {10.2458/azu_uapress_9780816531240-ch029},
	adsurl = {http://adsabs.harvard.edu/abs/2014prpl.conf..667B},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Baruteau_2016,
   title={Formation, Orbital and Internal Evolutions of Young Planetary Systems},
   volume={205},
   ISSN={1572-9672},
   url={http://dx.doi.org/10.1007/s11214-016-0258-z},
   DOI={10.1007/s11214-016-0258-z},
   number={1-4},
   journal={Space Science Reviews},
   publisher={Springer Science and Business Media LLC},
   author={Baruteau, Clément and Bai, Xuening and Mordasini, Christoph and Mollière, Paul},
   year={2016},
   month={May},
   pages={77–124}
}


@ARTICLE{Bitsch_2019a,
	author = {{Bitsch}, B. and {Izidoro}, A. and {Johansen}, A. and {Raymond}, S.~N. and 
	{Morbidelli}, A. and {Lambrechts}, M. and {Jacobson}, S.~A.},
	title = "{Formation of planetary systems by pebble accretion and migration: growth of gas giants}",
	journal = {aap},
	archivePrefix = "arXiv",
	eprint = {1902.08771},
	primaryClass = "astro-ph.EP",
	keywords = {accretion, accretion discs, planets and satellites: formation, protoplanetary discs, planet-disc interactions},
	year = 2019,
	month = mar,
	volume = 623,
	eid = {A88},
	pages = {A88},
	doi = {10.1051/0004-6361/201834489},
	adsurl = {http://adsabs.harvard.edu/abs/2019A%26A...623A..88B},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bitsch_2019b,
	author = {{Bitsch}, B. and {Raymond}, S.~N. and {Izidoro}, A.},
	title = "{Rocky super-Earths or waterworlds: the interplay of planet migration, pebble accretion, and disc evolution}",
	journal = {aap},
	archivePrefix = "arXiv",
	eprint = {1903.02488},
	primaryClass = "astro-ph.EP",
	keywords = {accretion, accretion disks, planets and satellites: formation, planets and satellites: composition, planet-disk interactions},
	year = 2019,
	month = apr,
	volume = 624,
	eid = {A109},
	pages = {A109},
	doi = {10.1051/0004-6361/201935007},
	adsurl = {http://adsabs.harvard.edu/abs/2019A%26A...624A.109B},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bondi_1944,
       author = {{Bondi}, H. and {Hoyle}, F.},
        title = "{On the mechanism of accretion by stars}",
      journal = {\mnras},
         year = "1944",
        month = "Jan",
       volume = {104},
        pages = {273},
          doi = {10.1093/mnras/104.5.273},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1944MNRAS.104..273B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bondi_1952,
	author = {{Bondi}, H.},
	title = "{On spherically symmetrical accretion}",
	journal = {mnras},
	year = 1952,
	volume = 112,
	pages = {195},
	doi = {10.1093/mnras/112.2.195},
	adsurl = {http://adsabs.harvard.edu/abs/1952MNRAS.112..195B},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Booth_2017,
   title={Chemical enrichment of giant planets and discs due to pebble drift},
   volume={469},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/stx1103},
   DOI={10.1093/mnras/stx1103},
   number={4},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Booth, Richard A. and Clarke, Cathie J. and Madhusudhan, Nikku and Ilee, John D.},
   year={2017},
   month={May},
   pages={3994–4011}
}

@article{Booth_2019,
   title={Planet-forming material in a protoplanetary disc: the interplay between chemical evolution and pebble drift},
   volume={487},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/stz1488},
   DOI={10.1093/mnras/stz1488},
   number={3},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Booth, R A and Ilee, J D},
   year={2019},
   month={May},
   pages={3998–4011}
}

@article{Bosman_2019,
   title={Jupiter formed as a pebble pile around the N2 ice line},
   volume={632},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/201936827},
   DOI={10.1051/0004-6361/201936827},
   journal={Astronomy \&Astrophysics},
   publisher={EDP Sciences},
   author={Bosman, A. D. and Cridland, A. J. and Miguel, Y.},
   year={2019},
   month={Dec},
   pages={L11}
}


@ARTICLE{Birnstiel_2010,
	author = {{Birnstiel}, T. and {Dullemond}, C.~P. and {Brauer}, F.},
	title = "{Gas- and dust evolution in protoplanetary disks}",
	journal = {aap},
	archivePrefix = "arXiv",
	eprint = {1002.0335},
	primaryClass = "astro-ph.EP",
	keywords = {accretion, accretion disks, circumstellar matter, stars: formation, stars: pre-main sequence, infrared: stars},
	year = 2010,
	month = apr,
	volume = 513,
	eid = {A79},
	pages = {A79},
	doi = {10.1051/0004-6361/200913731},
	adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...513A..79B},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Brogi_2019,
   title={Retrieving Temperatures and Abundances of Exoplanet Atmospheres with High-resolution Cross-correlation Spectroscopy},
   volume={157},
   ISSN={1538-3881},
   url={http://dx.doi.org/10.3847/1538-3881/aaffd3},
   DOI={10.3847/1538-3881/aaffd3},
   number={3},
   journal={The Astronomical Journal},
   publisher={American Astronomical Society},
   author={Brogi, Matteo and Line, Michael R.},
   year={2019},
   month={Feb},
   pages={114}
}

@ARTICLE{Cridland_2016,
	author = {{Cridland}, A.~J. and {Pudritz}, R.~E. and {Alessi}, M.},
	title = "{Composition of early planetary atmospheres - I. Connecting disc astrochemistry to the formation of planetary atmospheres}",
	journal = {mnras},
	archivePrefix = "arXiv",
	eprint = {1605.09407},
	primaryClass = "astro-ph.EP",
	keywords = {planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: formation, protoplanetary discs},
	year = 2016,
	month = sep,
	volume = 461,
	pages = {3274-3295},
	doi = {10.1093/mnras/stw1511},
	adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.461.3274C},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Cridland_2019,
   title={Connecting planet formation and astrochemistry},
   volume={627},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/201834378},
   DOI={10.1051/0004-6361/201834378},
   journal={Astronomy \&Astrophysics},
   publisher={EDP Sciences},
   author={Cridland, Alexander J. and Eistrup, Christian and van Dishoeck, Ewine F.},
   year={2019},
   month={Jul},
   pages={A127}
}

@article{Cridland_2020_vertical,
   title={Impact of vertical gas accretion on the carbon-to-oxygen ratio of gas giant atmospheres},
   volume={635},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/201936858},
   DOI={10.1051/0004-6361/201936858},
   journal={Astronomy \&Astrophysics},
   publisher={EDP Sciences},
   author={Cridland, Alexander J. and Bosman, Arthur D. and van Dishoeck, Ewine F.},
   year={2020},
   month={Mar},
   pages={A68}
}

@article{Cridland_2020_n2,
   title={Connecting planet formation and astrochemistry},
   volume={642},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/202038767},
   DOI={10.1051/0004-6361/202038767},
   journal={Astronomy \&Astrophysics},
   publisher={EDP Sciences},
   author={Cridland, Alex J. and van Dishoeck, Ewine F. and Alessi, Matthew and Pudritz, Ralph E.},
   year={2020},
   month={Oct},
   pages={A229}
}


@ARTICLE{Dodson-Robinson_2009,
	author = {{Dodson-Robinson}, Sarah E. and {Willacy}, Karen and
	{Bodenheimer}, Peter and {Turner}, Neal J. and {Beichman}, Charles A.},
	title = "{Ice lines, planetesimal composition and solid surface density in the solar nebula}",
	journal = {icarus},
	keywords = {Astrophysics},
	year = 2009,
	month = apr,
	volume = {200},
	number = {2},
	pages = {672-693},
	doi = {10.1016/j.icarus.2008.11.023},
	archivePrefix = {arXiv},
	eprint = {0806.3788},
	primaryClass = {astro-ph},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2009Icar..200..672D},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Eistrup_2018,
	author = {{Eistrup}, Christian and {Walsh}, Catherine and {van Dishoeck}, Ewine F.},
	title = "{Molecular abundances and C/O ratios in chemically evolving planet-forming disk midplanes}",
	journal = {aap},
	keywords = {protoplanetary disks, planets and satellites: formation, astrochemistry, planetary and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics},
	year = 2018,
	month = may,
	volume = {613},
	eid = {A14},
	pages = {A14},
	doi = {10.1051/0004-6361/201731302},
	archivePrefix = {arXiv},
	eprint = {1709.07863},
	primaryClass = {astro-ph.EP},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...613A..14E},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Giacobbe_2021,
   title={Five carbon- and nitrogen-bearing species in a hot giant planet’s atmosphere},
   volume={592},
   ISSN={1476-4687},
   url={http://dx.doi.org/10.1038/s41586-021-03381-x},
   DOI={10.1038/s41586-021-03381-x},
   number={7853},
   journal={Nature},
   publisher={Springer Science and Business Media LLC},
   author={Giacobbe, Paolo and Brogi, Matteo and Gandhi, Siddharth and Cubillos, Patricio E. and Bonomo, Aldo S. and Sozzetti, Alessandro and Fossati, Luca and Guilluy, Gloria and Carleo, Ilaria and Rainer, Monica and et al.},
   year={2021},
   month={Apr},
   pages={205–208}
}


@ARTICLE{Hartmann_1998,
	author = {{Hartmann}, Lee and {Calvet}, Nuria and {Gullbring}, Erik and
	{D'Alessio}, Paola},
	title = "{Accretion and the Evolution of T Tauri Disks}",
	journal = {\apj},
	keywords = {ACCRETION, ACCRETION DISKS, STARS: CIRCUMSTELLAR MATTER, STARS: FORMATION, STARS: PRE-MAIN-SEQUENCE, Accretion, Accretion Disks, Stars: Circumstellar Matter, Stars: Formation, Stars: Pre-Main-Sequence},
	year = 1998,
	month = mar,
	volume = {495},
	number = {1},
	pages = {385-400},
	doi = {10.1086/305277},
	adsurl = {https://ui.adsabs.harvard.edu/abs/1998ApJ...495..385H},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hasegawa_2019,
	author = {{Hasegawa}, Y. and {Hansen}, B.~M.~S. and {Vasisht}, G.},
	title = "{The Heavy-element Content Trend of Planets: A Tracer of their Formation Sites}",
	journal = {arXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1904.10288},
	primaryClass = "astro-ph.EP",
	keywords = {Astrophysics - Earth and Planetary Astrophysics},
	year = 2019,
	month = apr,
	adsurl = {http://adsabs.harvard.edu/abs/2019arXiv190410288H},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Helling_2014,
   title={Disk Evolution, Element Abundances and Cloud Properties of Young Gas Giant Planets},
   volume={4},
   ISSN={2075-1729},
   url={http://dx.doi.org/10.3390/life4020142},
   DOI={10.3390/life4020142},
   number={2},
   journal={Life},
   publisher={MDPI AG},
   author={Helling, Christiane and Woitke, Peter and Rimmer, Paul and Kamp, Inga and Thi, Wing-Fai and Meijerink, Rowin},
   year={2014},
   month={Apr},
   pages={142–173}
}

@article{Helling_2021,
   title={Cloud property trends in hot and ultra-hot giant gas planets (WASP-43b, WASP-103b, WASP-121b, HAT-P-7b, and WASP-18b)},
   volume={649},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/202039911},
   DOI={10.1051/0004-6361/202039911},
   journal={Astronomy & Astrophysics},
   publisher={EDP Sciences},
   author={Helling, Ch. and Lewis, D. and Samra, D. and Carone, L. and Graham, V. and Herbort, O. and Chubb, K. L. and Min, M. and Waters, R. and Parmentier, V. and et al.},
   year={2021},
   month={May},
   pages={A44}
}


@article{Hoeijmakers_2018,
   title={Atomic iron and titanium in the atmosphere of the exoplanet KELT-9b},
   volume={560},
   ISSN={1476-4687},
   url={http://dx.doi.org/10.1038/s41586-018-0401-y},
   DOI={10.1038/s41586-018-0401-y},
   number={7719},
   journal={Nature},
   publisher={Springer Science and Business Media LLC},
   author={Hoeijmakers, H. Jens and Ehrenreich, David and Heng, Kevin and Kitzmann, Daniel and Grimm, Simon L. and Allart, Romain and Deitrick, Russell and Wyttenbach, Aurélien and Oreshenko, Maria and Pino, Lorenzo and et al.},
   year={2018},
   month={Aug},
   pages={453–455}
}

@ARTICLE{Iaro_2007,
	author = {{Iaroslavitz}, Eyal and {Podolak}, Morris},
	title = "{Atmospheric mass deposition by captured planetesimals}",
	journal = {icarus},
	year = 2007,
	month = apr,
	volume = {187},
	number = {2},
	pages = {600-610},
	doi = {10.1016/j.icarus.2006.10.008},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2007Icar..187..600I},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Ida_2004,
   title={Toward a Deterministic Model of Planetary Formation. I. A Desert in the Mass and Semimajor Axis Distributions of Extrasolar Planets},
   volume={604},
   ISSN={1538-4357},
   url={http://dx.doi.org/10.1086/381724},
   DOI={10.1086/381724},
   number={1},
   journal={The Astrophysical Journal},
   publisher={American Astronomical Society},
   author={Ida, S. and Lin, D. N. C.},
   year={2004},
   month={Mar},
   pages={388–413}
}

@article{Ilee_2017,
   title={The chemistry of protoplanetary fragments formed via gravitational instabilities},
   volume={472},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/stx1966},
   DOI={10.1093/mnras/stx1966},
   number={1},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Ilee, J. D. and Forgan, D. H. and Evans, M. G. and Hall, C. and Booth, R. and Clarke, C. J. and Rice, W. K. M. and Boley, A. C. and Caselli, P. and Hartquist, T. W. and et al.},
   year={2017},
   month={Aug},
   pages={189–204}
}


@ARTICLE{Izidoro_2019,
	author = {{Izidoro}, A. and {Bitsch}, B. and {Raymond}, S.~N. and {Johansen}, A. and 
	{Morbidelli}, A. and {Lambrechts}, M. and {Jacobson}, S.~A.},
	title = "{Formation of planetary systems by pebble accretion and migration: Hot super-Earth systems from breaking compact resonant chains}",
	journal = {arXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1902.08772},
	primaryClass = "astro-ph.EP",
	keywords = {Astrophysics - Earth and Planetary Astrophysics},
	year = 2019,
	month = feb,
	adsurl = {http://adsabs.harvard.edu/abs/2019arXiv190208772I},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Kesseli_2021,
   title={Confirmation of Asymmetric Iron Absorption in WASP-76b with HARPS},
   volume={908},
   ISSN={2041-8213},
   url={http://dx.doi.org/10.3847/2041-8213/abe047},
   DOI={10.3847/2041-8213/abe047},
   number={1},
   journal={The Astrophysical Journal},
   publisher={American Astronomical Society},
   author={Kesseli, Aurora Y. and Snellen, I. A. G.},
   year={2021},
   month={Feb},
   pages={L17}
}

@ARTICLE{Lecar_2006,
	author = {{Lecar}, M. and {Podolak}, M. and {Sasselov}, D. and {Chiang}, E.},
	title = "{On the Location of the Snow Line in a Protoplanetary Disk}",
	journal = {\apj},
	keywords = {Stars: Planetary Systems: Formation, Stars: Planetary Systems: Protoplanetary Disks, Astrophysics},
	year = 2006,
	month = apr,
	volume = {640},
	number = {2},
	pages = {1115-1118},
	doi = {10.1086/500287},
	archivePrefix = {arXiv},
	eprint = {astro-ph/0602217},
	primaryClass = {astro-ph},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...640.1115L},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lambrechts_2019,
	author = {{Lambrechts}, M. and {Morbidelli}, A. and {Jacobson}, S.~A. and 
	{Johansen}, A. and {Bitsch}, B. and {Izidoro}, A. and {Raymond}, S.~N.
	},
	title = "{Formation of planetary systems by pebble accretion and migration: How the radial pebble flux determines a terrestrial-planet or super-Earth growth mode}",
	journal = {arXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1902.08694},
	primaryClass = "astro-ph.EP",
	keywords = {Astrophysics - Earth and Planetary Astrophysics},
	year = 2019,
	month = feb,
	adsurl = {http://adsabs.harvard.edu/abs/2019arXiv190208694L},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Lissauer_2009,
	author = {{Lissauer}, Jack J. and {Hubickyj}, Olenka and {D'Angelo}, Gennaro and
	{Bodenheimer}, Peter},
	title = "{Models of Jupiter's growth incorporating thermal and hydrodynamic constraints}",
	journal = {icarus},
	keywords = {Astrophysics},
	year = 2009,
	month = feb,
	volume = {199},
	number = {2},
	pages = {338-350},
	doi = {10.1016/j.icarus.2008.10.004},
	archivePrefix = {arXiv},
	eprint = {0810.5186},
	primaryClass = {astro-ph},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2009Icar..199..338L},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lodders_2009,
	author = {{Lodders}, K. and {Palme}, H.},
	title = "{Solar System Elemental Abundances in 2009}",
	journal = {Meteoritics and Planetary Science Supplement},
	year = 2009,
	month = sep,
	volume = 72,
	pages = {5154},
	adsurl = {http://adsabs.harvard.edu/abs/2009M%26PSA..72.5154L},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Lozovsky_2017,
	author = {{Lozovsky}, Michael and {Helled}, Ravit and {Rosenberg}, Eric D. and
	{Bodenheimer}, Peter},
	title = "{Jupiter{\textquoteright}s Formation and Its Primordial Internal Structure}",
	journal = {\apj},
	keywords = {planets and satellites: composition, planets and satellites: formation, planets and satellites: gaseous planets, planets and satellites: individual: Jupiter, planets and satellites: interiors, Astrophysics - Earth and Planetary Astrophysics},
	year = 2017,
	month = feb,
	volume = {836},
	number = {2},
	eid = {227},
	pages = {227},
	doi = {10.3847/1538-4357/836/2/227},
	archivePrefix = {arXiv},
	eprint = {1701.01719},
	primaryClass = {astro-ph.EP},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...836..227L},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Machida_2010,
   author = {{Machida}, M.~N. and {Kokubo}, E. and {Inutsuka}, S.-I. and 
	{Matsumoto}, T.},
    title = "{Gas accretion onto a protoplanet and formation of a gas giant planet}",
  journal = {mnras},
archivePrefix = "arXiv",
   eprint = {1002.3002},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, hydrodynamics, planets and satellites: formation, Solar system: formation, planetary systems},
     year = 2010,
    month = jun,
   volume = 405,
    pages = {1227-1243},
      doi = {10.1111/j.1365-2966.2010.16527.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.405.1227M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{Madhusudhan_2014,
	title={TOWARD CHEMICAL CONSTRAINTS ON HOT JUPITER MIGRATION},
	volume={794},
	ISSN={2041-8213},
	url={http://dx.doi.org/10.1088/2041-8205/794/1/L12},
	DOI={10.1088/2041-8205/794/1/l12},
	number={1},
	journal={The Astrophysical Journal},
	publisher={IOP Publishing},
	author={Madhusudhan, Nikku and Amin, Mustafa A. and Kennedy, Grant M.},
	year={2014},
	month={Sep},
	pages={L12}
}

@article{Madhusudhan_2017,
    author = {Pinhas, Arazi and Madhusudhan, Nikku and Clarke, Cathie},
    title = "{Efficiency of planetesimal ablation in giant planetary envelopes}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {463},
    number = {4},
    pages = {4516-4532},
    year = {2016},
    month = {09},
    abstract = "{Observations of exoplanetary spectra are leading to unprecedented constraints on their atmospheric elemental abundances, particularly O/H, C/H, and C/O ratios. Recent studies suggest that elemental ratios could provide important constraints on formation and migration mechanisms of giant exoplanets. A fundamental assumption in such studies is that the chemical composition of the planetary envelope represents the sum-total of compositions of the accreted gas and solids during the formation history of the planet. We investigate the efficiency with which accreted planetesimals ablate in a giant planetary envelope thereby contributing to its composition rather than sinking to the core. From considerations of aerodynamic drag causing ‘frictional ablation’ and the envelope temperature structure causing ‘thermal ablation’, we compute mass ablations for impacting planetesimals of radii 30 m to 1 km for different compositions (ice to iron) and a wide range of velocities and impact angles, assuming spherical symmetry. Icy impactors are fully ablated in the outer envelope for a wide range of parameters. Even for Fe impactors substantial ablation occurs in the envelope for a wide range of sizes and velocities. For example, iron impactors of sizes below ∼0.5 km and velocities above ∼30 km s−1 are found to ablate by ∼60–80 per cent within the outer envelope at pressures below 103 bar due to frictional ablation alone. For deeper pressures (∼107 bar), substantial ablation happens over a wider range of parameters. Therefore, our exploratory study suggests that atmospheric abundances of volatile elements in giant planets reflect their accretion history during formation.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stw2239},
    url = {https://doi.org/10.1093/mnras/stw2239},
    eprint = {https://academic.oup.com/mnras/article-pdf/463/4/4516/18513317/stw2239.pdf},
}


@ARTICLE{Min_2010,
   author = {{Min}, M. and {Dullemond}, C.~P. and {Kama}, M. and {Dominik}, C.
	},
    title = "{The thermal structure and the location of the snow line in the protosolar nebula: Axisymmetric models with full 3-D radiative transfer}",
  journal = {Icarus},
archivePrefix = "arXiv",
   eprint = {1012.0727},
 primaryClass = "astro-ph.EP",
     year = 2011,
    month = mar,
   volume = 212,
    pages = {416-426},
      doi = {10.1016/j.icarus.2010.12.002},
   adsurl = {http://adsabs.harvard.edu/abs/2011Icar..212..416M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Machida_2010,
	author = {{Machida}, Masahiro N. and {Kokubo}, Eiichiro and
	{Inutsuka}, Shu-Ichiro and {Matsumoto}, Tomoaki},
	title = "{Gas accretion onto a protoplanet and formation of a gas giant planet}",
	journal = {Monthly Notices of the Royal Astronomy Society},
	keywords = {accretion, accretion discs, hydrodynamics, planets and satellites: formation, Solar system: formation, planetary systems, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
	year = "2010",
	month = "Jun",
	volume = {405},
	number = {2},
	pages = {1227-1243},
	doi = {10.1111/j.1365-2966.2010.16527.x},
	archivePrefix = {arXiv},
	eprint = {1002.3002},
	primaryClass = {astro-ph.SR},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.405.1227M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Mordasini_2016,
	title={THE IMPRINT OF EXOPLANET FORMATION HISTORY ON OBSERVABLE PRESENT-DAY SPECTRA OF HOT JUPITERS},
	volume={832},
	ISSN={1538-4357},
	url={http://dx.doi.org/10.3847/0004-637X/832/1/41},
	DOI={10.3847/0004-637x/832/1/41},
	number={1},
	journal={The Astrophysical Journal},
	publisher={American Astronomical Society},
	author={Mordasini, C. and van Boekel, R. and Mollière, P. and Henning, Th. and Benneke, Björn},
	year={2016},
	month={Nov},
	pages={41}
}

@article{Molliere_2020,
   title={Retrieving scattering clouds and disequilibrium chemistry in the atmosphere of HR 8799e},
   volume={640},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/202038325},
   DOI={10.1051/0004-6361/202038325},
   journal={Astronomy \&Astrophysics},
   publisher={EDP Sciences},
   author={Mollière, P. and Stolker, T. and Lacour, S. and Otten, G. P. P. L. and Shangguan, J. and Charnay, B. and Molyarova, T. and Nowak, M. and Henning, Th. and Marleau, G.-D. and et al.},
   year={2020},
   month={Aug},
   pages={A131}
}


@article{Mordasini_2017,
   title={Characterization of exoplanets from their formation},
   volume={608},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/201630077},
   DOI={10.1051/0004-6361/201630077},
   journal={Astronomy \&Astrophysics},
   publisher={EDP Sciences},
   author={Mordasini, C. and Marleau, G.-D. and Mollière, P.},
   year={2017},
   month={Dec},
   pages={A72}
}


@article{Mordasini_2018,
   title={Planetary Population Synthesis},
   ISBN={9783319553337},
   url={http://dx.doi.org/10.1007/978-3-319-55333-7_143},
   DOI={10.1007/978-3-319-55333-7_143},
   journal={Handbook of Exoplanets},
   publisher={Springer International Publishing},
   author={Mordasini, Christoph},
   year={2018},
   pages={2425–2474}
}


@article{Notsu_2020,
   title={The composition of hot Jupiter atmospheres assembled within chemically evolved protoplanetary discs},
   volume={499},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/staa2944},
   DOI={10.1093/mnras/staa2944},
   number={2},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Notsu, Shota and Eistrup, Christian and Walsh, Catherine and Nomura, Hideko},
   year={2020},
   month={Sep},
   pages={2229–2244}
}

@article{Oberg_2011,
   title={THE EFFECTS OF SNOWLINES ON C/O IN PLANETARY ATMOSPHERES},
   volume={743},
   ISSN={2041-8213},
   url={http://dx.doi.org/10.1088/2041-8205/743/1/L16},
   DOI={10.1088/2041-8205/743/1/l16},
   number={1},
   journal={The Astrophysical Journal},
   publisher={IOP Publishing},
   author={\"{O}berg, Karin I. and Murray-Clay, Ruth and Bergin, Edwin A.},
   year={2011},
   month={Nov},
   pages={L16}
}

@article{Oberg_2016,
   title={EXCESS C/O AND C/H IN OUTER PROTOPLANETARY DISK GAS},
   volume={831},
   ISSN={2041-8213},
   url={http://dx.doi.org/10.3847/2041-8205/831/2/L19},
   DOI={10.3847/2041-8205/831/2/l19},
   number={2},
   journal={The Astrophysical Journal},
   publisher={American Astronomical Society},
   author={Öberg, Karin I. and Bergin, Edwin A.},
   year={2016},
   month={Nov},
   pages={L19}
}


@ARTICLE{Oberg_2020,
	author = {{Oberg}, Karin I. and {Bergin}, Edwin A.},
	title = "{Astrochemistry and compositions of planetary systems}",
	journal = {arXiv e-prints},
	keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
	year = 2020,
	month = oct,
	eid = {arXiv:2010.03529},
	pages = {arXiv:2010.03529},
	archivePrefix = {arXiv},
	eprint = {2010.03529},
	primaryClass = {astro-ph.EP},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201003529O},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{Otten_2020,
      title={Direct characterization of young giant exoplanets at high spectral resolution by coupling SPHERE and CRIRES+}, 
      author={G. P. P. L. Otten and A. Vigan and E. Muslimov and M. N'Diaye and E. Choquet and U. Seemann and K. Dohlen and M. Houllé and P. Cristofari and M. W. Phillips and Y. Charles and I. Baraffe and J. -L. Beuzit and A. Costille and R. Dorn and M. El Morsy and M. Kasper and M. Lopez and C. Mordasini and R. Pourcelot and A. Reiners and J. -F. Sauvage},
      year={2020},
      eprint={2009.01841},
      archivePrefix={arXiv},
      primaryClass={astro-ph.IM}
}

@article{Pekmezci_2020,
	doi = {10.3847/1538-4357/abbd90},
	url = {https://doi.org/10.3847/1538-4357/abbd90},
	year = 2020,
	month = {nov},
	publisher = {American Astronomical Society},
	volume = {904},
	number = {2},
	pages = {129},
	author = {G. S. Pekmezci and O. Mousis and J. I. Lunine},
	title = {Planetary Refractory Composition and Volatile Accretion into Gas Giants in the Protoplanetary Disks of the Sun and {WASP}-12},
	journal = {The Astrophysical Journal},
	abstract = {We present a detailed theoretical exploration of the refractory compositions and volatile enrichments of planets forming in protoplanetary disks with solar-like conditions. The two cases of the Sun and WASP-12 are studied due to the availability of spectral measurements and their known planets. The distribution throughout their disks of solid compounds with a wide range of volatilities is computed by a comprehensive chemical thermodynamics code. After the calculation of refractory compounds down to the water snowline, the compositional distributions are documented for planets generated in certain locations of protoplanetary disks depending on thermodynamic conditions. These results are referred to proposed bulk compositions for solar terrestrial planets, and for the core of the hot Jupiter WASP-12b. The material left over after the formation of rocky components is collected and treated in calculations to determine the abundances of fundamental volatile molecules in the outer regions of the disks. The distributions of planetesimal volatile composition are then altered for four different cases of the carbon-to-oxygen ratios, and for oxidizing and reducing conditions, in order to adjust the best fit for the accretion zone of Jupiter and WASP-12b. We compare the Jovian results to in situ atmospheric measurements from Jupiter’s atmosphere. Overall, this study proposes a holistic approach to estimate possible planetary interior and envelope compositions from hot toward cold disk zones, along with the mass of planetesimals accreted into the envelopes of gas giants.}
}


@ARTICLE{Piso_2014a,
	author = {{Piso}, A.-M.~A. and {Youdin}, A.~N. and {Murray-Clay}, R.~A.
	},
	title = "{Minimum Core Masses for Giant Planet Formation with Realistic Equations of State and Opacities}",
	journal = {apj},
	archivePrefix = "arXiv",
	eprint = {1412.5185},
	primaryClass = "astro-ph.EP",
	keywords = {planets and satellites: atmospheres, planets and satellites: formation, planets and satellites: gaseous planets },
	year = 2015,
	month = feb,
	volume = 800,
	eid = {82},
	pages = {82},
	doi = {10.1088/0004-637X/800/2/82},
	adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...800...82P},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Piso_2014b,
	author = {{Piso}, A.-M.~A. and {Youdin}, A.~N.},
	title = "{On the Minimum Core Mass for Giant Planet Formation at Wide Separations}",
	journal = {apj},
	archivePrefix = "arXiv",
	eprint = {1311.0011},
	primaryClass = "astro-ph.EP",
	keywords = {planets and satellites: atmospheres, planets and satellites: formation, planets and satellites: gaseous planets},
	year = 2014,
	month = may,
	volume = 786,
	eid = {21},
	pages = {21},
	doi = {10.1088/0004-637X/786/1/21},
	adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...786...21P},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Piso_2016,
   title={THE ROLE OF ICE COMPOSITIONS FOR SNOWLINES AND THE C/N/O RATIOS IN ACTIVE DISKS},
   volume={833},
   ISSN={1538-4357},
   url={http://dx.doi.org/10.3847/1538-4357/833/2/203},
   DOI={10.3847/1538-4357/833/2/203},
   number={2},
   journal={The Astrophysical Journal},
   publisher={American Astronomical Society},
   author={Piso, Ana-Maria A. and Pegues, Jamila and Öberg, Karin I.},
   year={2016},
   month={Dec},
   pages={203}
}


@ARTICLE{Podolak_1988,
       author = {{Podolak}, M. and {Pollack}, J.~B. and {Reynolds}, R.~T.},
        title = "{Interactions of planetesimals with protoplanetary atmospheres}",
      journal = {icarus},
     keywords = {Giant Stars, Planetary Atmospheres, Planetary Evolution, Planetary Mass, Protoplanets, Solar Corona, Computational Astrophysics, High Temperature, Molecular Weight, Planetary Cores, PLANETS, INTERACTIONS, PLANETESIMALS, ATMOSPHERE, GIANT PLANETS, CORE, FORMATION, ACCRETION, GRAVITY EFFECTS, GASES, SOLAR NEBULA, CAPTURE, CALCULATIONS, TWO-BODY PROBLEM, TRAJECTORIES, DRAG, MASS, DEPTH, SIZE, ICY BODIES, ROCKY BODIES, COMPOSITION, THEORETICAL STUDIES, NUMERICAL METHODS, PARAMETERS, MODELS, ANGULAR MOMENTUM, COMPARISONS, Lunar and Planetary Exploration; Planets},
         year = 1988,
        month = jan,
       volume = {73},
       number = {1},
        pages = {163-179},
          doi = {10.1016/0019-1035(88)90090-5},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988Icar...73..163P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Podolak_2020,
   title={Detailed Calculations of the Efficiency of Planetesimal Accretion in the Core-accretion Model},
   volume={899},
   ISSN={1538-4357},
   url={http://dx.doi.org/10.3847/1538-4357/ab9ec1},
   DOI={10.3847/1538-4357/ab9ec1},
   number={1},
   journal={The Astrophysical Journal},
   publisher={American Astronomical Society},
   author={Podolak, Morris and Haghighipour, Nader and Bodenheimer, Peter and Helled, Ravit and Podolak, Esther},
   year={2020},
   month={Aug},
   pages={45}
}


@ARTICLE{Pollack_1996,
       author = {{Pollack}, James B. and {Hubickyj}, Olenka and {Bodenheimer}, Peter and
         {Lissauer}, Jack J. and {Podolak}, Morris and {Greenzweig}, Yuval},
        title = "{Formation of the Giant Planets by Concurrent Accretion of Solids and Gas}",
      journal = {icarus},
         year = 1996,
        month = nov,
       volume = {124},
       number = {1},
        pages = {62-85},
          doi = {10.1006/icar.1996.0190},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996Icar..124...62P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Pudritz_2018_rev,
   title={Connecting Planetary Composition with Formation},
   ISBN={9783319553337},
   url={http://dx.doi.org/10.1007/978-3-319-55333-7_144},
   DOI={10.1007/978-3-319-55333-7_144},
   journal={Handbook of Exoplanets},
   publisher={Springer International Publishing},
   author={Pudritz, Ralph E. and Cridland, Alex J. and Alessi, Matthew},
   year={2018},
   pages={2475–2521}
}

@article{Santos_2017,
   title={Constraining planet structure and composition from stellar chemistry: trends in different stellar populations},
   volume={608},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/201731359},
   DOI={10.1051/0004-6361/201731359},
   journal={Astronomy \&Astrophysics},
   publisher={EDP Sciences},
   author={Santos, N. C. and Adibekyan, V. and Dorn, C. and Mordasini, C. and Noack, L. and Barros, S. C. C. and Delgado-Mena, E. and Demangeon, O. and Faria, J. P. and Israelian, G. and et al.},
   year={2017},
   month={Dec},
   pages={A94}
}

@article{Serindag_2021,
   title={Is TiO emission present in the ultra-hot Jupiter WASP-33b? A reassessment using the improved ExoMol TOTO line list},
   volume={645},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/202039135},
   DOI={10.1051/0004-6361/202039135},
   journal={Astronomy \&Astrophysics},
   publisher={EDP Sciences},
   author={Serindag, Dilovan B. and Nugroho, Stevanus K. and Mollière, Paul and de Mooij, Ernst J. W. and Gibson, Neale P. and Snellen, Ignas A. G.},
   year={2021},
   month={Jan},
   pages={A90}
}

@article{Shibata_2020,
   title={The origin of the high metallicity of close-in giant exoplanets},
   volume={633},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/201936700},
   DOI={10.1051/0004-6361/201936700},
   journal={Astronomy \&Astrophysics},
   publisher={EDP Sciences},
   author={Shibata, Sho and Helled, Ravit and Ikoma, Masahiro},
   year={2020},
   month={Jan},
   pages={A33}
}


@ARTICLE{Siess_2000,
	author = {{Siess}, L. and {Dufour}, E. and {Forestini}, M.},
	title = "{An internet server for pre-main sequence tracks of low- and intermediate-mass stars}",
	journal = {aap},
	keywords = {EQUATION OF STATE, STARS: EVOLUTION, STARS: HERTZSPRUNG-RUSSEL (HR) AND C-M DIAGRAMS, STARS: PRE-MAIN SEQUENCE, ASTRONOMICAL DATA BASES: MISCELLANEOUS, Astrophysics},
	year = 2000,
	month = jun,
	volume = {358},
	pages = {593-599},
	archivePrefix = {arXiv},
	eprint = {astro-ph/0003477},
	primaryClass = {astro-ph},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...358..593S},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Snellen_2010,
   title={The orbital motion, absolute mass and high-altitude winds of exoplanet HD-209458b},
   volume={465},
   ISSN={1476-4687},
   url={http://dx.doi.org/10.1038/nature09111},
   DOI={10.1038/nature09111},
   number={7301},
   journal={Nature},
   publisher={Springer Science and Business Media LLC},
   author={Snellen, Ignas A. G. and de Kok, Remco J. and de Mooij, Ernst J. W. and Albrecht, Simon},
   year={2010},
   month={Jun},
   pages={1049–1051}
}

@article{Thiabaud_2015,
   title={Elemental ratios in stars vs planets},
   volume={580},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/201525963},
   DOI={10.1051/0004-6361/201525963},
   journal={Astronomy \&Astrophysics},
   publisher={EDP Sciences},
   author={Thiabaud, Amaury and Marboeuf, Ulysse and Alibert, Yann and Leya, Ingo and Mezger, Klaus},
   year={2015},
   month={Jul},
   pages={A30}
}

@article{Thorngren_2016,
   title={THE MASS–METALLICITY RELATION FOR GIANT PLANETS},
   volume={831},
   ISSN={1538-4357},
   url={http://dx.doi.org/10.3847/0004-637X/831/1/64},
   DOI={10.3847/0004-637x/831/1/64},
   number={1},
   journal={The Astrophysical Journal},
   publisher={American Astronomical Society},
   author={Thorngren, Daniel P. and Fortney, Jonathan J. and Murray-Clay, Ruth A. and Lopez, Eric D.},
   year={2016},
   month={Oct},
   pages={64}
}

@article{Turrini_2020,
   title={Tracing the Formation History of Giant Planets in Protoplanetary Disks with Carbon, Oxygen, Nitrogen, and Sulfur},
   volume={909},
   ISSN={1538-4357},
   url={http://dx.doi.org/10.3847/1538-4357/abd6e5},
   DOI={10.3847/1538-4357/abd6e5},
   number={1},
   journal={The Astrophysical Journal},
   publisher={American Astronomical Society},
   author={Turrini, D. and Schisano, E. and Fonte, S. and Molinari, S. and Politi, R. and Fedele, D. and Panić, O. and Kama, M. and Changeat, Q. and Tinetti, G.},
   year={2021},
   month={Mar},
   pages={40}
}

@ARTICLE{Venturini_2016,
	author = {{Venturini}, Julia and {Alibert}, Yann and {Benz}, Willy},
	title = "{Planet formation with envelope enrichment: new insights on planetary diversity}",
	journal = {aap},
	keywords = {planets and satellites: formation, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics},
	year = 2016,
	month = dec,
	volume = {596},
	eid = {A90},
	pages = {A90},
	doi = {10.1051/0004-6361/201628828},
	archivePrefix = {arXiv},
	eprint = {1609.00960},
	primaryClass = {astro-ph.EP},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...596A..90V},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Visser_2011,
	author = {{Visser}, R. and {Doty}, S.~D. and {van Dishoeck}, E.~F.},
	title = "{The chemical history of molecules in circumstellar disks. II. Gas-phase species}",
	journal = {aap},
	keywords = {astrochemistry, stars: formation, circumstellar matter, protoplanetary disks, molecular processes, Astrophysics - Astrophysics of Galaxies},
	year = 2011,
	month = oct,
	volume = {534},
	eid = {A132},
	pages = {A132},
	doi = {10.1051/0004-6361/201117249},
	archivePrefix = {arXiv},
	eprint = {1109.1741},
	primaryClass = {astro-ph.GA},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...534A.132V},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Voelkel_2020,
   title={Effect of pebble flux-regulated planetesimal formation on giant planet formation},
   volume={642},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/202038085},
   DOI={10.1051/0004-6361/202038085},
   journal={Astronomy \&Astrophysics},
   publisher={EDP Sciences},
   author={Voelkel, Oliver and Klahr, Hubert and Mordasini, Christoph and Emsenhuber, Alexandre and Lenz, Christian},
   year={2020},
   month={Oct},
   pages={A75}
}

@ARTICLE{Woitke_2018,
	author = {{Woitke}, P. and {Helling}, C. and {Hunter}, G.~H. and {Millard}, J.~D. and 
	{Turner}, G.~E. and {Worters}, M. and {Blecic}, J. and {Stock}, J.~W.
	},
	title = "{Equilibrium chemistry down to 100 K. Impact of silicates and phyllosilicates on the carbon to oxygen ratio}",
	journal = {aap},
	archivePrefix = "arXiv",
	eprint = {1712.01010},
	primaryClass = "astro-ph.EP",
	keywords = {astrochemistry, planets and satellites: atmospheres, planets and satellites: composition, stars: winds, outflows, molecular data, methods: numerical},
	year = 2018,
	month = jun,
	volume = 614,
	eid = {A1},
	pages = {A1},
	doi = {10.1051/0004-6361/201732193},
	adsurl = {http://adsabs.harvard.edu/abs/2018A%26A...614A...1W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Zinzi_2017,
   title={Anti-correlation between multiplicity and orbital properties  in exoplanetary systems as a possible record   of their dynamical histories},
   volume={605},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/201731595},
   DOI={10.1051/0004-6361/201731595},
   journal={Astronomy \&Astrophysics},
   publisher={EDP Sciences},
   author={Zinzi, A. and Turrini, D.},
   year={2017},
   month={Sep},
   pages={L4}
}





